Identifying the Complete Correlation Structure in Large-Scale High-Dimensional Data Sets with Local False Discovery Rates

The identification of the dependent components in multiple data sets is a fundamental problem in many practical applications. The challenge in these applications is that often the data sets are high-dimensional with few observations or available samples and contain latent components with unknown probability distributions. A novel mathematical formulation of this problem is proposed, which enables the inference of the underlying correlation structure with strict false positive control. In particular, the false discovery rate is controlled at a pre-defined threshold on two levels simultaneously. The deployed test statistics originate in the sample coherence matrix. The required probability models are learned from the data using the bootstrap. Local false discovery rates are used to solve the multiple hypothesis testing problem. Compared to the existing techniques in the literature, the developed technique does not assume an a priori correlation structure and work well when the number of data sets is large while the number of observations is small. In addition, it can handle the presence of distributional uncertainties, heavy-tailed noise, and outliers.

==> sections/fund.tex <==
\section{Fundamentals \textit{TO BE RENAMED}}
\label{sec:fund}
	\subsection{Multiple Hypothesis Testing}
	\label{sec:fund_mht}
		\begin{itemize}
			\item Motivate multiple testing
			\item Introduce the \gls{fdr}
		\end{itemize}

==> sections/int.tex <==
\section{Introduction}
\label{sec:int}


	\textbf{Goal}: In this work, we aim to identify the underling correlation structure structure of the components across multiple data sets.\\
	\textbf{Contribution}: A novel, robust procedure to identify the correlation structure using the eigenvalue decomposition of the coherence matrix using multiple hypothesis testing and the bootstrap. Works well especially in the small sample case. The false discovery rate is controlled, which allows to assess the significance of the inference results. We propose tailored decision making algorithms that take the specific structure of the problem into account.
	
	\textbf{Bullet points for Introduction:}
	
	\begin{itemize}
		\item Motivation - Applications of analyzing multivariate second-order association among different data sets in fusion of data from different brain imaging modalities \cite{Akhonda2021}, genomics, wireless acoustic sensor networks \cite{Hasija2019a}, finding biomarkers in epilepsy \cite{} etc. 

		\item Tools - Various tools exist, Matrix decomposition methods like IVA, factor analysis, CCA and its multiset extension are well-suited as they limit model search space to avoid overfitting and at the same time rely on minimal assumptions on the latent components \cite{} 

		\item CCA and its extensions extract maximally correlated components between different data sets and these are then used in the applications mentioned above [Hotelling, Kettenring,15,16 in Sigpro paper]. Even nonlinear extensions of CCA such as deep CCA extract highly correlated components after applying a highly-complex nonlinear transforming on the original data by the use of neural networks [Andrew,Wang].     
		
		\item One of the simplifying assumptions is that the extracted components are same for all sets, i.e., are common to all sets like [Wu, Hovine] or are correlated across all sets like [Hasija SSP 2016]. However, this is restrictive for numerous applications like brain imaging data fusion where data sets correspond to different modalities and some modalities are closely related and thus have more correlated components than other pair of modalities. E.g., fmri and sMRI are both MRI modalities while sMRI and EEG are completely different. 
		
		\item Thus, estimating the correlation structure is necessary to fully characterize the second-order association across the data sets [Sigpro paper]. 
		
		\item An introductory example, similar to \cite[Fig.~1]{Hasija2020}

		\item State-of-the-art - Largely focused on model-order selection \cite{}, this is not sufficient for more than two data set, previous work on correlation structure estimation involved performing pairwise hypothesis tests \cite{} and joint approach \cite{}. In [Siddique], the authors estimate the structure using the results from [Sigpro] and applied it to estimate the structure of each set of extracted components one by one using an IVA model. However, all of these work rely on having lots of samples. 
		
		%None of the previous work addressed FDR control. 
	
		\item Limited sample size issue - Correlation among extracted components is overestimated, leads to a problem to not knowing which components are actually correlated with each other, this gets exacerbated as the number of data sets increase, leads to false interpretation in applications - talk about issue of interpretability in fMRI data fusion, asymptotic results do not work well, giving an idea about noisy/spurious correlations 
		
		\item False discoveries - Another issue, Again connecting it to our particular and other applications in how an uncontrolled FDR could lead to false discoveries of activated brain regions 
		
		\item Our proposed approach - The benefits are three fold. We tackle limited sample regime, provide FDR control and is scalable for large number of data sets. 
	\end{itemize}
 %show benefits by solving a real-world problem which is important in brain imaging data fusion. 
 Our method is based on theoretical proves using random matrix theory and proposes novel empirical solutions for practical purposes.  

